MetaScientist: A Human-AI Synergistic Framework for Automated Mechanical Metamaterial Design

The discovery of novel mechanical metamaterials, whose properties are dominated by their engineered structures rather than chemical composition, is a knowledge-intensive and resource-demanding process. To accelerate the design of novel metamaterials, we present MetaScientist, a human-in-the-loop system that integrates advanced AI capabilities with expert oversight with two primary phases: (1) hypothesis generation, where the system performs complex reasoning to generate novel and scientifically sound hypotheses, supported with domain-specific foundation models and inductive biases retrieved from existing literature; (2) 3D structure synthesis, where a 3D structure is synthesized with a novel 3D diffusion model based on the textual hypothesis and refined it with a LLM-based refinement model to achieve better structure properties. At each phase, domain experts iteratively validate the system outputs, and provide feedback and supplementary materials to ensure the alignment of the outputs with scientific principles and human preferences. Through extensive evaluation from human scientists, MetaScientist is able to deliver novel and valid mechanical metamaterial designs that have the potential to be highly impactful in the metamaterial field.

==> sections/3case_study_backup.tex <==
\section{Case Study and Experiments}
\label{sec:case_study}

\minqian{move the description of example after each method section; if there's any, for important components including foundation model (2.2), hypothesis generation (2.3), 3D diffusion model (2.4), hypothesis refinement model (2.5), add (1) training dataset statistics and (2) quantitative evaluation results }
% \jy{TODO: zian}
\subsection{Task Formulation} 

To demonstrate the capability of the developed pipeline in generating hypotheses and corresponding lattice metamaterials for solving specific research problems, design tasks are carefully chosen based on three principles, i.e., significance, realism, and testability. One such example is the classical weight minimization problem, in our context, design a lattice material for structure support using minimum material. Such problems are common and well-studied in engineering, materials science, and biology, as reducing the structure weight brings significant economic benefits (reduced material and energy costs). 
%As shown schematically in Fig. x, 
The design space is set as a 5 cm cube and the target weight is 10 kg. To enable the generation of detailed lattice structure, we further assign the composition material as a polymer with modulus of 20 GPa and strength of 5 MPa. The input research question is: 
\textit{Let's design a 3D printed lattice structure for supporting weights. The weight is 10 kg and the lattice structure is about 5 cm in size. The material is polymer with modulus of 20 GPa and strength of 50 MPa. Please design a periodic lattice structure with minimum material usage.}

The demonstration example also showcases the different functional panels of the interface, including human-LLM interaction, hypotheses based lattice structure generation using the trained diffusion model, visualization, and fine tuning.


% \subsection{Human-in-the-Loop Feedback}

% The roles that human scientists play in the human-LLM synergistic hypothesis generation include: 1) Define research question and choosing the direction of hypothesis formulation - this ensures on-demand hypothesis generation; 2) Provide knowledge and relevant papers in the high-level hypothesis generation - sparkling diverse initial hypothesis; 3) Fact check, monitoring the generated results and correct errors - this ensures the accuracy and reliability of the result; 4) Implementation and validation. By involving humans in these aspects, we leverage the strengths of LLMs while ensuring that hypotheses are customized, novel, reliable, and tailored to solve real-world problems.

\subsection{Demonstration example}

Our demonstration example follows the six-step interface in hypothesis generation (see the demo video). In the first step, the user defines the research question as discussed above. In the second step, the user provides feedback and relevant research papers to help refine the hypothesis interactively. Note that in some cases, our fine-tuned LLMs can generate satisfactory high-level ideas without human feedback (e.g., our fine-tuned LLaMA-3.1 model directly proposes the usage of octet lattice to achieve high structural efficiency). In contrast, general purpose models like GPT-4o need human feedback to improve the hypothesis - with hinting prompts like \textit{“Please consider the most efficient lattice structures, particularly those known for high stiffness and strength.” }, GPT-4o proposes using octet lattice. Step three searches for relevant research papers and extracts inductive bias, these information is displayed as knowledge snippets, and the human scientist can easily add or remove the snippets. In our example, two research papers on octet lattice were provided while less relevant information on atomic lattice and structural buckling were removed. 

Stage four further refines the high-level hypothesis into specific, measurable details by providing the mechanical properties of the lattice including Young's modulus, shear modulus, and Poisson's ratio in three orthogonal directions. Notably, while the generated mechanical properties are in the reasonable range, they do not satisfy the symmetry requirement. As such, human feedback is provided: \textit{“Octet lattice is a cubic material, there are constraints on its modulus and Poisson's ratio
%For instance, the three Young's modulus should be the same.
...” } The model learns the information and generates the property matrix correctly. 
In step five, our diffusion model successfully generates the octet lattice based on the hypothesis and property matrix, displays the unit cell and the corresponding mechanical properties. In the final step, the user can add constrains and optimization goals for the generated lattice structure. This process combines a customized language model and a developed numerical homogenization pipeline, ensuring the reliability of the structural design. Moreover, both the unit cells of the original and refined lattices are displayed, highlighting structural changes made in the refinement process. Explanations of what aspects have been improved in the refined unit cell such as connectivity, geometry, stiffness, etc are also provided.

% Propmpts:
% Let's design a 3D printed lattice structure for supporting weights. The weight is 10 kg and the lattice structure is about 5 cm in size. The material is polymer with modulus of 20 GPa and strength of 50 MPa. Please design a periodic lattice structure with minimum material usage. 

% Please use the most efficient lattice structures, e.g., lattice structures that are known for high stiffness and strength. 

% Octet is a nice choice. Please further estimate what is the strength of the lattice material that is needed to safely support the weight. Based on which estimate the expected relative density of the lattice material that is needed. Please refer to the provided reference for detailing the design. 

% Octet lattice is a cubic material, there are constraints on its modulus and Poisson's ratio. For instance, the three Young's modulus should be the same. In addition, the strength of the lattice should be considered in finalizing the design, since we want the lattice to be safely supporting a weight. 

\subsection{Results and validation}

The octet unit cell design generated by our developed pipeline for weight support is shown in Fig. x, which has a relative modulus (Ex, Ey, and Ez) of 0.016 and a relative density of 0.0705. Octet is one of the well-known strong structures and can be considered as the correct answer to our question. Our theoretical estimation also suggests that this lattice structure is capable to support weight >30 kg. Interacting with model through the chat interface suggests that the model followed the basic principles in structure generation - relying on a stretching-dominant mechanism for mechanical efficiency and generating unit cells using scale relationship, and knows that a safety factor 
%in the range of 3~5 
is important to guarantee safe deployment. We printed the lattice using a 3D printer (Formlab 3) and the resultant is shown capable to support 10 kg weight reliably, validating the application of the developed pipeline in solving real-world problems.


==> sections/Methods/overview.tex <==
\subsection{Overview}

Our \system{} system aims to produce a textual novel hypothesis associated with a validated and refined 3D lattice structure given the research question input by the user. \system{} consists of three primary phases. \textbf{First}, \textit{hypothesis generation} takes the user's research question as input and produces a natural language hypothesis and lattice properties. \textbf{Second}, we use a \textit{3D structure generation} module to produce a 3D metamaterial design based on the previously generated lattice properties. \textbf{Finally}, we employ a \textit{hypothesis refinement } stage to iteratively refine the hypothetical 3D structure into a more valid and effective structure.

In each phase, human users can provide various types of feedback through the interface to iteratively improve the system's output and then proceed to the next phase when they are satisfied. This human-in-the-loop mechanism enables the user to have flexible and fine-grained control over the generation and refinement process, making the generated hypotheses and 3D structures more valid, creative, and aligned with user requirements.\minqian{done}
% \minqian{stages + human in the loop. each stage will incorporate specific feedback to address their distinct challenge. }

==> sections/intro_backup.tex <==
\section{Introduction}
\label{sec:introduction}

% Metamaterials, an interdisciplinary research area involving materials science, physics, and many other fields, focuses on artificially engineered structures that exhibit unique properties not found in natural materials.

Metamaterials are microstructured material whose material properties go beyond those of the ingredient materials, often possessing unusual mechanical and/or functional properties.  The advancements in metamaterials have fostered a vast amount of technological innovations across various key domains, such as infrastructure, transportation, and information technology\zian{ applications-need adjustment}. 
However, scientists are facing two critical challenges in designing and discovering metamaterials.

First, the design of metamaterials is \textit{knowledge-intensive}, relying heavily on human intuition, creativity, and a deep understanding of complex scientific principles. As the field expands exponentially, it becomes increasingly challenging for researchers to keep pace with the rapid accumulation of knowledge. For instance, the number of metamaterial-related publications has grown from 156 papers in 2000 to over 30,000 papers in 2023\zian{7170 in 2010}, with approximately Z new papers published monthly~\cite{}\jy{TODO: number of xyz}. This massive expansion leads to significant barriers to effectively accessing, synthesizing, and applying the vast body of research, ultimately slowing the pace of technological innovation.

Second, the development process is \textit{resource-intensive}. Traditional metamaterial development pipelines involve multiple time-consuming stages, including conceptualization, theoretical modeling, experimentation, and computational simulation. Each stage requires significant human, financial, and computational resources. The relative isolation of research efforts and the inherent complexity of design processes further limit researchers’ ability to efficiently explore and validate new metamaterial concepts, constraining both research throughput and scalability.

To tackle these challenges, we introduce \system{}, a multi-phase human-in-the-loop system for assisting and accelerating novel metamaterial design by leveraging large language models (LLMs) and diffusion models. As depicted in Figure~\ref{}, \system{} comprises three key phases: \textbf{(1) Hypothesis Generation}: given an input research question, we perform abductive and recursive reasoning upon evidence and inductive biases retrieved from a large 
% By retrieving and processing material science literature, we derive inductive biases and employ a metamaterial domain-specific foundation model to conduct abductive, recursive, and evidence-based reasoning, generating innovative hypotheses. 
\textbf{(2) 3D Structure Generation}: The generated hypotheses are transformed into 3D metamaterial structures, which are then subjected to computational simulations to validate their physical properties. \textbf{(3) 3D Structure Refinement}: Utilizing numerical and verbal reinforcement learning, the system iteratively refines both the hypotheses and the corresponding structures, further enhancing accuracy and performance.

Additionally, \system{} incorporates a human-in-the-loop mechanism to mitigate potential limitations of LLMs, such as hallucinations and reliance on outdated information. While LLMs excel at knowledge synthesis and reasoning, domain experts provide cutting-edge insights, iterative feedback, and error correction at each phase of the system. This expert oversight ensures that the generated hypotheses are scientifically sound and align with the latest advances in the field.

In summary, we propose \system{}, a semi-autonomous hypothesis-generation framework that bridges the gap between computational capabilities and human expertise. By integrating retrieval-augmented generation, reinforcement learning, and human oversight, \system{} significantly reduces resource dependencies while accelerating research efficiency in metamaterial discovery. Through its robust hypothesis-generation pipeline and simulation capabilities, our system offers a scalable solution to the challenges of metamaterial design.

% Metamaterials, characterized by properties derived from their engineered structures rather than chemical compositions, have revolutionized technological innovation, enabling breakthroughs in sensing, information technology, infrastructure, and transportation. However, their design and discovery remain constrained by two critical challenges: knowledge-intensiveness and resource-intensiveness.

% Designing metamaterials relies heavily on expert intuition, creativity, and a deep understanding of complex scientific principles. As metamaterials research grows exponentially, scientists increasingly struggle to keep up with advancements, leading to significant challenges in accessing and effectively applying this vast body of knowledge. At the same time, traditional metamaterial development processes, including conceptualization, theoretical modeling, experimentation, and computational simulations, require substantial human, financial, and computational resources. This resource-intensive nature slows down innovation and limits scalability.

% Recent advancements in artificial intelligence (AI), particularly large foundation models that can synthesize vast amounts of research knowledge and generate innovative insights, offer a promising solution to the challenges of knowledge and resource intensiveness in metamaterial design. These models provide unprecedented capabilities to navigate and process complex information, enabling the rapid generation of creative hypotheses. Motivated by the potential to address these barriers, we propose \system{}, a semi-autonomous framework designed to revolutionize the metamaterial design process. By leveraging the strengths of large language models (LLMs), advanced computational reasoning, and bio-inspired design principles, \system{} offers a transformative approach to automating and accelerating the discovery of novel metamaterials, bridging the gap between human expertise and AI-driven innovation.

% The \system{} framework comprises three key phases: (1) \textit{Hypothesis Generation}, where abductive, recursive, and evidence-based reasoning is applied to material science literature to generate innovative ideas; (2) \textit{3D Structure Generation}, transforming hypotheses into 3D metamaterial structures and validating their performance through advanced simulations; and (3) \textit{Hypothesis Refinement}, utilizing numerical and verbal reinforcement learning to iteratively improve both hypotheses and their corresponding structures. To further enhance effectiveness, \system{} adapts LLMs to seamlessly process unstructured natural language and structured scientific data, supported by a human-in-the-loop mechanism for iterative feedback and error correction.

% A distinguishing feature of \system{} is its ability to autonomously derive inductive biases from scientific literature, enabling the generation of novel, cost-efficient, and creative hypotheses at scale. Moreover, inspired by intricate lattice structures found in biological systems, the framework incorporates bio-inspired designs as a source of innovation. This synergy of hypothesis-driven reasoning, automated validation, and iterative refinement bridges the gap between computational power and expert judgment, significantly reducing resource dependence and accelerating research efficiency.

% This work presents the conceptual foundation, technical innovations, and envisioned impact of \system{}, illustrating how this AI-driven framework embodies principles of creativity, skepticism, and scalability to redefine metamaterial design and unlock unprecedented possibilities across scientific domains.

% \section{intro2}
% Metamaterials, defined by their engineered structures rather than their chemical compositions, have emerged as a frontier in disruptive technologies, enabling unprecedented possibilities in domains such as sensing, information technology, infrastructure, and transportation~\cite{}. However, the design and discovery of metamaterials face two critical challenges that hinder progress.

% The first challenge is \textit{knowledge-intensiveness}. Designing metamaterials is an expertise-driven process that relies heavily on human intuition, creativity, and deep understanding of complex scientific principles. As the volume of research on metamaterials expands exponentially, it becomes increasingly difficult for scientists to keep pace with the latest advancements, leading to bottlenecks in accessing and applying this vast body of knowledge effectively.

% The second challenge is \textit{resource-intensiveness}. Traditional metamaterial development pipelines involve multiple time-consuming stages, including conceptualization, theoretical modeling, experimentation, and computational simulations. These stages require significant human, financial, and computational resources, which constrain research throughput and slow the pace of innovation.

% On the other hand, recent advancements in large foundation models, particularly their ability to process vast amounts of research literature, synthesize knowledge, and generate creative insights, offer a promising avenue to overcome these barriers. Inspired by this progress, we propose \system{}, a semi-autonomous computational system designed to integrate advanced AI capabilities with expert oversight to revolutionize the metamaterial design pipeline.
% As illustrated in Figure~\ref{}, \system{} comprises three key phases:
% \textbf{Hypothesis Generation}: Given a research question or topic, \system{} employs abductive, recursive, and evidence-based reasoning grounded in material science literature to formulate innovative hypotheses.
% \textbf{3D Structure Generation}: Hypotheses are transformed into 3D metamaterial structures, followed by simulations to evaluate their physical properties and performance metrics.
% \textbf{Hypothesis Refinement}: Through numerical and verbal reinforcement learning, \system{} iteratively refines both the hypotheses and their corresponding 3D structures, guided by feedback from domain experts.
% In addition, to equip \system{} with specialized knowledge in material science, we adapt large language models (LLMs) to process both unstructured natural language and structured data seamlessly. While these LLMs excel in synthesizing and reasoning, they are prone to limitations such as hallucinations, outdated information, and misalignment with human preferences. To address these issues, we incorporate a human-in-the-loop mechanism into the workflow. Domain experts provide iterative feedback at each phase, validating hypotheses, correcting errors, proposing specific requirements, and contributing cutting-edge knowledge to guide the model’s innovation trajectory.

% In summary, \system{} bridges the gap between computational power and expert judgment, leveraging retrieval-augmented generation, reinforcement learning, and human oversight to accelerate metamaterial discovery. By integrating simulation capabilities with a robust hypothesis-generation pipeline, \system{} significantly reduces dependence on human resources and improves research efficiency.
